Variational Variance: Simple, Reliable, Calibrated Heteroscedastic Noise Variance Parameterization

Brittle optimization has been observed to adversely impact model likelihoods for regression and VAEs when simultaneously fitting neural network mappings from a (random) variable onto the mean and variance of a dependent Gaussian variable. Previous works have bolstered optimization and improved likelihoods, but fail other basic posterior predictive checks (PPCs). Under the PPC framework, we propose critiques to test predictive mean and variance calibration and the predictive distribution's ability to generate sensible data. We find that our attractively simple solution, to treat heteroscedastic variance variationally, sufficiently regularizes variance to pass these PPCs. We consider a diverse gamut of existing and novel priors and find our methods preserve or outperform existing model likelihoods while significantly improving parameter calibration and sample quality for regression and VAEs.

==> assets/generative_table.tex <==
\begin{tabular}{llllll}
\toprule
      &            &                           LL &                     Mean RMSE &                      Var Bias &                   Sample RMSE \\
Dataset & Method &                              &                               &                               &                               \\
\midrule
fashion mnist & Fixed-Var. VAE (1.0) &             -730.05$\pm$0.11 &              0.15$\pm$1.8e-03 &              0.98$\pm$5.7e-04 &              1.01$\pm$3.7e-04 \\
      & Fixed-Var. VAE (0.001) &            -1452.44$\pm$3.65 &  \textbf{9.4e-02$\pm$4.6e-05} &          -7.8e-03$\pm$8.6e-06 &  \textbf{9.9e-02$\pm$4.7e-05} \\
      & VAE &            2154.31$\pm$42.11 &              0.25$\pm$1.4e-03 &           3.3e-02$\pm$1.5e-03 &              0.39$\pm$3.1e-03 \\
      & VAE + BN &            1639.39$\pm$15.33 &              0.20$\pm$1.8e-03 &           2.1e-02$\pm$3.0e-03 &              0.31$\pm$5.6e-03 \\
      & VAE-Split &            2099.28$\pm$39.97 &              0.27$\pm$2.9e-03 &           4.7e-02$\pm$1.6e-03 &              0.45$\pm$4.8e-03 \\
      & VAE-Split + BN &            1948.30$\pm$25.87 &              0.26$\pm$6.2e-03 &           3.1e-02$\pm$3.6e-03 &              0.41$\pm$1.1e-02 \\
      & Detlefsen &         -1624.12$\pm$8.3e-03 &              0.16$\pm$8.2e-04 &              9.97$\pm$3.3e-04 &              3.17$\pm$1.2e-03 \\
      & MAP-VAE &            1003.51$\pm$32.75 &              0.11$\pm$4.1e-03 &          -9.1e-03$\pm$6.2e-04 &              0.13$\pm$4.8e-03 \\
      & Student-VAE &   \textbf{3134.52$\pm$18.60} &              0.29$\pm$3.3e-03 &           7.4e-02$\pm$1.6e-02 &              0.49$\pm$2.2e-02 \\
      & V3AE-VAP &            2146.46$\pm$67.83 &              0.28$\pm$3.5e-03 &  \textbf{9.9e-04$\pm$3.0e-03} &              0.40$\pm$8.2e-03 \\
      & V3AE-Gamma &            1201.95$\pm$25.25 &              0.11$\pm$2.8e-03 &          -8.0e-03$\pm$4.1e-04 &              0.12$\pm$3.4e-03 \\
      & V3AE-VAMP &            1632.22$\pm$12.89 &              0.17$\pm$1.3e-03 &           1.5e-03$\pm$2.7e-04 &              0.25$\pm$2.4e-03 \\
      & V3AE-VAMP* &            1630.10$\pm$17.87 &              0.18$\pm$2.6e-03 &           1.3e-03$\pm$2.5e-04 &              0.25$\pm$3.4e-03 \\
      & V3AE-xVAMP &            1601.60$\pm$21.49 &              0.18$\pm$2.5e-03 &           1.3e-03$\pm$4.1e-04 &              0.25$\pm$3.8e-03 \\
      & V3AE-xVAMP* &            1619.97$\pm$25.95 &              0.18$\pm$3.3e-03 &           1.5e-03$\pm$4.6e-04 &              0.25$\pm$5.0e-03 \\
      & V3AE-VBEM &              306.46$\pm$1.04 &              0.10$\pm$6.8e-04 &           6.4e-02$\pm$9.7e-05 &              0.29$\pm$3.3e-04 \\
      & V3AE-VBEM* &             1153.11$\pm$4.20 &              0.10$\pm$5.5e-04 &  \textbf{4.4e-04$\pm$3.9e-05} &              0.15$\pm$8.0e-04 \\
mnist & Fixed-Var. VAE (1.0) &             -732.10$\pm$0.11 &              0.17$\pm$1.1e-03 &              0.98$\pm$4.2e-04 &              1.02$\pm$2.5e-04 \\
      & Fixed-Var. VAE (0.001) &           -2902.66$\pm$29.23 &     \textbf{0.11$\pm$3.3e-04} &          -1.2e-02$\pm$7.4e-05 &     \textbf{0.12$\pm$3.1e-04} \\
      & VAE &           2593.51$\pm$267.72 &              0.25$\pm$2.7e-03 &           4.3e-02$\pm$2.6e-02 &              0.41$\pm$3.5e-02 \\
      & VAE + BN &            2386.70$\pm$23.17 &              0.25$\pm$1.8e-03 &              0.13$\pm$2.6e-02 &              0.50$\pm$2.6e-02 \\
      & VAE-Split &            2282.32$\pm$65.63 &              0.25$\pm$2.7e-03 &           7.4e-02$\pm$2.6e-02 &              0.44$\pm$3.2e-02 \\
      & VAE-Split + BN &            2482.36$\pm$75.34 &              0.28$\pm$4.4e-03 &           6.2e-02$\pm$1.1e-02 &              0.47$\pm$1.5e-02 \\
      & Detlefsen &            -1561.89$\pm$1.36 &              0.18$\pm$6.7e-04 &              9.12$\pm$2.1e-02 &              3.03$\pm$3.2e-03 \\
      & MAP-VAE &             1291.42$\pm$6.94 &              0.13$\pm$1.9e-03 &          -1.3e-02$\pm$4.1e-04 &              0.15$\pm$2.0e-03 \\
      & Student-VAE &  \textbf{4826.82$\pm$530.95} &              0.27$\pm$1.7e-02 &                 0.38$\pm$0.45 &                 0.68$\pm$0.28 \\
      & V3AE-VAP &           3243.11$\pm$445.47 &              0.24$\pm$3.5e-03 &  \textbf{8.1e-04$\pm$9.7e-04} &              0.34$\pm$5.5e-03 \\
      & V3AE-Gamma &             1495.01$\pm$2.75 &              0.13$\pm$7.0e-04 &          -1.2e-02$\pm$1.9e-04 &              0.15$\pm$9.2e-04 \\
      & V3AE-VAMP &            2355.12$\pm$13.40 &              0.20$\pm$6.7e-04 &  \textbf{6.2e-04$\pm$1.1e-03} &              0.28$\pm$1.7e-03 \\
      & V3AE-VAMP* &            2270.76$\pm$41.89 &              0.20$\pm$7.9e-04 &  \textbf{1.2e-03$\pm$1.1e-03} &              0.29$\pm$2.2e-03 \\
      & V3AE-xVAMP &            2323.38$\pm$94.35 &              0.20$\pm$2.6e-03 &  \textbf{1.9e-03$\pm$6.8e-04} &              0.29$\pm$3.2e-03 \\
      & V3AE-xVAMP* &            2280.13$\pm$48.29 &              0.20$\pm$2.0e-03 &  \textbf{6.5e-04$\pm$7.2e-04} &              0.29$\pm$3.7e-03 \\
      & V3AE-VBEM &              296.95$\pm$0.92 &              0.12$\pm$8.1e-04 &           6.1e-02$\pm$2.7e-04 &              0.30$\pm$2.7e-04 \\
      & V3AE-VBEM* &             2107.63$\pm$5.44 &              0.14$\pm$1.2e-03 &  \textbf{1.6e-03$\pm$1.1e-04} &              0.20$\pm$1.6e-03 \\
\bottomrule
\end{tabular}



==> assets/generative_table_mnist.tex <==
\begin{tabular}{lllll}
\toprule
{} &                           LL &                  Mean RMSE &                      Var Bias &                Sample RMSE \\
Method                 &                              &                            &                               &                            \\
\midrule
Fixed-Var. VAE (1.0)   &             -732.10$\pm$0.11 &           0.17$\pm$1.1e-03 &              0.98$\pm$4.2e-04 &           1.02$\pm$2.5e-04 \\
Fixed-Var. VAE (0.001) &           -2902.66$\pm$29.23 &  \textbf{0.11$\pm$3.3e-04} &          -1.2e-02$\pm$7.4e-05 &  \textbf{0.12$\pm$3.1e-04} \\
VAE                    &           2593.51$\pm$267.72 &           0.25$\pm$2.7e-03 &           4.3e-02$\pm$2.6e-02 &           0.41$\pm$3.5e-02 \\
VAE + BN               &            2386.70$\pm$23.17 &           0.25$\pm$1.8e-03 &              0.13$\pm$2.6e-02 &           0.50$\pm$2.6e-02 \\
VAE-Split              &            2282.32$\pm$65.63 &           0.25$\pm$2.7e-03 &           7.4e-02$\pm$2.6e-02 &           0.44$\pm$3.2e-02 \\
VAE-Split + BN         &            2482.36$\pm$75.34 &           0.28$\pm$4.4e-03 &           6.2e-02$\pm$1.1e-02 &           0.47$\pm$1.5e-02 \\
Detlefsen              &            -1561.89$\pm$1.36 &           0.18$\pm$6.7e-04 &              9.12$\pm$2.1e-02 &           3.03$\pm$3.2e-03 \\
MAP-VAE                &             1291.42$\pm$6.94 &           0.13$\pm$1.9e-03 &          -1.3e-02$\pm$4.1e-04 &           0.15$\pm$2.0e-03 \\
Student-VAE            &  \textbf{4826.82$\pm$530.95} &           0.27$\pm$1.7e-02 &                 0.38$\pm$0.45 &              0.68$\pm$0.28 \\
V3AE-VAP               &           3243.11$\pm$445.47 &           0.24$\pm$3.5e-03 &  \textbf{8.1e-04$\pm$9.7e-04} &           0.34$\pm$5.5e-03 \\
V3AE-Gamma             &             1495.01$\pm$2.75 &           0.13$\pm$7.0e-04 &          -1.2e-02$\pm$1.9e-04 &           0.15$\pm$9.2e-04 \\
V3AE-VAMP              &            2355.12$\pm$13.40 &           0.20$\pm$6.7e-04 &  \textbf{6.2e-04$\pm$1.1e-03} &           0.28$\pm$1.7e-03 \\
V3AE-VAMP*             &            2270.76$\pm$41.89 &           0.20$\pm$7.9e-04 &  \textbf{1.2e-03$\pm$1.1e-03} &           0.29$\pm$2.2e-03 \\
V3AE-xVAMP             &            2323.38$\pm$94.35 &           0.20$\pm$2.6e-03 &  \textbf{1.9e-03$\pm$6.8e-04} &           0.29$\pm$3.2e-03 \\
V3AE-xVAMP*            &            2280.13$\pm$48.29 &           0.20$\pm$2.0e-03 &  \textbf{6.5e-04$\pm$7.2e-04} &           0.29$\pm$3.7e-03 \\
V3AE-VBEM              &              296.95$\pm$0.92 &           0.12$\pm$8.1e-04 &           6.1e-02$\pm$2.7e-04 &           0.30$\pm$2.7e-04 \\
V3AE-VBEM*             &             2107.63$\pm$5.44 &           0.14$\pm$1.2e-03 &  \textbf{1.6e-03$\pm$1.1e-04} &           0.20$\pm$1.6e-03 \\
\bottomrule
\end{tabular}



==> assets/regression_uci_mean_bias.tex <==
\begin{tabular}{lllllll}
\toprule
             &       &                   boston &                        carbon &                   concrete &                  energy &                          naval \\
Algorithm & Prior& (506, 13, 1)& (10721, 5, 3)& (1030, 8, 1)& (768, 8, 2)& (11934, 16, 2)\\
\midrule
Detlefsen & N/A &           -0.67$\pm$1.81 &          -9.8e-04$\pm$3.5e-03 &             -0.03$\pm$3.30 &           0.15$\pm$0.87 &           -2.8e-04$\pm$6.3e-04 \\
Normal & N/A &           -0.28$\pm$0.56 &           5.5e-05$\pm$2.1e-04 &              0.32$\pm$0.66 &           0.06$\pm$0.10 &           -1.3e-04$\pm$1.2e-04 \\
Student & N/A &           -0.50$\pm$0.51 &          -4.3e-05$\pm$1.4e-04 &             -0.04$\pm$0.72 &          -0.06$\pm$0.13 &           -1.0e-04$\pm$1.5e-04 \\
Gamma-Normal & VAP &           -0.31$\pm$0.54 &           1.5e-04$\pm$2.2e-04 &              0.06$\pm$0.73 &          -0.03$\pm$0.12 &           -4.1e-05$\pm$8.1e-05 \\
             & Standard &           -0.39$\pm$0.67 &           5.0e-05$\pm$1.9e-04 &              0.09$\pm$0.72 &           0.04$\pm$0.10 &           -1.4e-04$\pm$8.5e-05 \\
             & VAMP &  \textbf{-0.18$\pm$0.52} &  \textbf{9.5e-06$\pm$2.3e-04} &             -0.10$\pm$0.58 &  \textbf{0.02$\pm$0.11} &           -4.6e-06$\pm$5.5e-05 \\
             & VAMP* &           -0.18$\pm$0.52 &           7.9e-05$\pm$2.0e-04 &             -0.10$\pm$0.58 &           0.02$\pm$0.11 &           -8.9e-06$\pm$6.0e-05 \\
             & xVAMP &           -0.25$\pm$0.54 &           4.6e-05$\pm$1.8e-04 &  \textbf{9.2e-03$\pm$0.63} &           0.03$\pm$0.11 &  \textbf{-1.8e-06$\pm$7.1e-05} \\
             & xVAMP* &           -0.24$\pm$0.54 &           1.3e-04$\pm$2.0e-04 &              0.03$\pm$0.66 &           0.02$\pm$0.11 &            3.8e-06$\pm$6.2e-05 \\
             & VBEM &           -0.18$\pm$0.54 &           7.3e-05$\pm$3.8e-04 &             -0.01$\pm$0.55 &           0.03$\pm$0.11 &            1.5e-05$\pm$2.8e-05 \\
             & VBEM* &           -0.19$\pm$0.58 &          -2.2e-05$\pm$2.1e-04 &             -0.02$\pm$0.63 &           0.03$\pm$0.11 &            1.9e-05$\pm$5.8e-05 \\
\midrule
             &       &                power plant &       superconductivity &                    wine-red &                 wine-white &                    yacht \\
Algorithm & Prior& (9568, 4, 1)& (21263, 81, 1)& (1599, 11, 1)& (4898, 11, 1)& (308, 6, 1)\\
\midrule
Detlefsen & N/A &              0.15$\pm$0.79 &           1.22$\pm$3.11 &               0.02$\pm$0.12 &  \textbf{2.8e-03$\pm$0.08} &  \textbf{-0.06$\pm$1.19} \\
Normal & N/A &          -9.9e-03$\pm$0.07 &           0.90$\pm$0.62 &  \textbf{-5.1e-03$\pm$0.06} &          -3.3e-03$\pm$0.03 &           -0.96$\pm$0.82 \\
Student & N/A &              0.06$\pm$0.08 &           0.29$\pm$0.54 &              -0.07$\pm$0.06 &             -0.02$\pm$0.03 &           -7.47$\pm$2.71 \\
Gamma-Normal & VAP &              0.02$\pm$0.05 &          -0.08$\pm$0.33 &              -0.01$\pm$0.06 &          -7.0e-03$\pm$0.03 &           -7.22$\pm$2.74 \\
             & Standard &          -9.6e-03$\pm$0.11 &           0.74$\pm$0.33 &              -0.02$\pm$0.06 &             -0.01$\pm$0.03 &           -5.42$\pm$1.86 \\
             & VAMP &           3.2e-03$\pm$0.06 &           0.09$\pm$0.38 &              -0.01$\pm$0.06 &             -0.01$\pm$0.03 &           -0.62$\pm$1.53 \\
             & VAMP* &           3.2e-03$\pm$0.06 &           0.06$\pm$0.39 &              -0.01$\pm$0.06 &             -0.01$\pm$0.03 &           -0.60$\pm$1.53 \\
             & xVAMP &           6.5e-03$\pm$0.07 &          -0.03$\pm$0.41 &           -9.6e-03$\pm$0.06 &          -7.9e-03$\pm$0.03 &           -5.44$\pm$2.46 \\
             & xVAMP* &           2.0e-03$\pm$0.06 &  \textbf{0.01$\pm$0.49} &           -8.8e-03$\pm$0.06 &          -8.7e-03$\pm$0.03 &           -5.59$\pm$2.61 \\
             & VBEM &           1.2e-03$\pm$0.10 &           0.25$\pm$0.45 &           -9.6e-03$\pm$0.06 &          -5.8e-03$\pm$0.03 &           -0.17$\pm$0.52 \\
             & VBEM* &  \textbf{3.0e-05$\pm$0.07} &           0.09$\pm$0.46 &           -9.2e-03$\pm$0.06 &          -7.6e-03$\pm$0.02 &           -2.00$\pm$1.30 \\
\bottomrule
\end{tabular}



==> assets/regression_uci_mean_rmse.tex <==
\begin{tabular}{lllllll}
\toprule
             &       &                  boston &                        carbon &                concrete &                  energy &                         naval \\
Algorithm & Prior& (506, 13, 1)& (10721, 5, 3)& (1030, 8, 1)& (768, 8, 2)& (11934, 16, 2)\\
\midrule
\cite{sun2019functional} & N/A & \textit{2.38$\pm$0.10} & -- & \textit{4.94$\pm$0.18} & \textit{0.41$\pm$0.02} & \textit{1.2e-04$\pm$0.00} \\
Detlefsen & N/A &           4.48$\pm$1.06 &              0.02$\pm$4.6e-03 &           8.13$\pm$1.65 &           2.05$\pm$0.49 &           4.2e-03$\pm$6.3e-04 \\
Normal & N/A &           3.36$\pm$1.29 &  \textbf{7.5e-03$\pm$3.3e-03} &           6.05$\pm$0.66 &           1.30$\pm$0.14 &           3.5e-03$\pm$3.1e-04 \\
Student & N/A &           3.62$\pm$1.42 &           7.6e-03$\pm$3.3e-03 &           6.71$\pm$0.81 &           1.42$\pm$0.17 &           3.4e-03$\pm$5.0e-04 \\
Gamma-Normal & VAP &           3.44$\pm$1.21 &           7.7e-03$\pm$3.3e-03 &           6.61$\pm$0.84 &           1.38$\pm$0.15 &           3.2e-03$\pm$5.3e-04 \\
             & Standard &           3.82$\pm$1.72 &           7.6e-03$\pm$3.3e-03 &           6.63$\pm$0.70 &           1.31$\pm$0.14 &           3.2e-03$\pm$5.1e-04 \\
             & VAMP &           3.15$\pm$1.06 &           7.8e-03$\pm$3.2e-03 &           5.47$\pm$1.00 &           1.36$\pm$0.13 &           1.2e-03$\pm$1.0e-03 \\
             & VAMP* &           3.15$\pm$1.05 &           7.8e-03$\pm$3.2e-03 &           5.47$\pm$1.00 &           1.36$\pm$0.13 &           1.6e-03$\pm$1.3e-03 \\
             & xVAMP &           3.25$\pm$1.16 &           7.6e-03$\pm$3.3e-03 &           5.61$\pm$0.67 &           1.36$\pm$0.14 &           3.2e-03$\pm$5.2e-04 \\
             & xVAMP* &           3.28$\pm$1.17 &           7.6e-03$\pm$3.3e-03 &           5.72$\pm$0.59 &           1.36$\pm$0.14 &           3.2e-03$\pm$4.9e-04 \\
             & VBEM &  \textbf{3.14$\pm$1.07} &           8.7e-03$\pm$3.3e-03 &  \textbf{5.26$\pm$0.58} &           1.36$\pm$0.14 &  \textbf{5.6e-04$\pm$1.6e-04} \\
             & VBEM* &           3.18$\pm$1.12 &           7.6e-03$\pm$3.3e-03 &           5.59$\pm$0.70 &  \textbf{1.30$\pm$0.13} &           2.4e-03$\pm$2.8e-04 \\
\midrule
             &       &             power plant &        superconductivity &                wine-red &              wine-white &                   yacht \\
Algorithm & Prior& (9568, 4, 1)& (21263, 81, 1)& (1599, 11, 1)& (4898, 11, 1)& (308, 6, 1)\\
\midrule
\cite{sun2019functional} & N/A & \textit{4.10$\pm$0.05} & -- & -- & -- & \textit{0.61$\pm$0.07} \\
Detlefsen & N/A &           4.33$\pm$0.27 &           17.72$\pm$1.29 &           0.71$\pm$0.06 &           0.76$\pm$0.04 &  \textbf{2.42$\pm$1.06} \\
Normal & N/A &  \textbf{4.12$\pm$0.20} &           14.53$\pm$0.44 &           0.62$\pm$0.03 &           0.70$\pm$0.04 &           3.42$\pm$2.30 \\
Student & N/A &           4.12$\pm$0.19 &           14.85$\pm$0.42 &           0.63$\pm$0.03 &           0.71$\pm$0.03 &          15.03$\pm$3.30 \\
Gamma-Normal & VAP &           4.14$\pm$0.21 &           14.83$\pm$0.48 &           0.62$\pm$0.03 &           0.70$\pm$0.03 &          14.70$\pm$3.31 \\
             & Standard &           4.18$\pm$0.18 &           14.44$\pm$0.43 &           0.63$\pm$0.03 &           0.72$\pm$0.03 &          12.17$\pm$2.38 \\
             & VAMP &           4.16$\pm$0.20 &           12.81$\pm$0.33 &           0.62$\pm$0.03 &           0.70$\pm$0.04 &           5.42$\pm$3.54 \\
             & VAMP* &           4.16$\pm$0.20 &  \textbf{12.80$\pm$0.35} &           0.62$\pm$0.03 &           0.70$\pm$0.04 &           5.30$\pm$3.65 \\
             & xVAMP &           4.14$\pm$0.20 &           14.13$\pm$0.39 &           0.62$\pm$0.03 &           0.70$\pm$0.04 &          12.30$\pm$3.09 \\
             & xVAMP* &           4.13$\pm$0.21 &           14.25$\pm$0.42 &           0.62$\pm$0.03 &           0.70$\pm$0.03 &          12.51$\pm$3.20 \\
             & VBEM &           4.16$\pm$0.19 &           13.13$\pm$0.37 &  \textbf{0.62$\pm$0.03} &  \textbf{0.69$\pm$0.03} &           3.51$\pm$1.46 \\
             & VBEM* &           4.12$\pm$0.19 &           14.08$\pm$0.42 &           0.62$\pm$0.03 &           0.69$\pm$0.03 &           5.33$\pm$2.58 \\
\bottomrule
\end{tabular}



==> assets/regression_uci_rmse.tex <==
\begin{tabular}{lllllll}
\toprule
             &       &                  boston &                        carbon &                concrete &                  energy &                         naval \\
Algorithm & Prior& (506, 13, 1)& (10721, 5, 3)& (1030, 8, 1)& (768, 8, 2)& (11934, 16, 2)\\
\midrule
Detlefsen & N/A &           4.48$\pm$1.06 &              0.02$\pm$4.6e-03 &           8.13$\pm$1.65 &           2.05$\pm$0.49 &           4.2e-03$\pm$6.3e-04 \\
Normal & N/A &           3.36$\pm$1.29 &  \textbf{7.5e-03$\pm$3.3e-03} &           6.05$\pm$0.66 &           1.30$\pm$0.14 &           3.5e-03$\pm$3.1e-04 \\
Student & N/A &           3.62$\pm$1.42 &           7.6e-03$\pm$3.3e-03 &           6.71$\pm$0.81 &           1.42$\pm$0.17 &           3.4e-03$\pm$5.0e-04 \\
Gamma-Normal & VAP &           3.44$\pm$1.21 &           7.7e-03$\pm$3.3e-03 &           6.61$\pm$0.84 &           1.38$\pm$0.15 &           3.2e-03$\pm$5.3e-04 \\
             & Standard &           3.82$\pm$1.72 &           7.6e-03$\pm$3.3e-03 &           6.63$\pm$0.70 &           1.31$\pm$0.14 &           3.2e-03$\pm$5.1e-04 \\
             & VAMP &           3.15$\pm$1.06 &           7.8e-03$\pm$3.2e-03 &           5.47$\pm$1.00 &           1.36$\pm$0.13 &           1.2e-03$\pm$1.0e-03 \\
             & VAMP* &           3.15$\pm$1.05 &           7.8e-03$\pm$3.2e-03 &           5.47$\pm$1.00 &           1.36$\pm$0.13 &           1.6e-03$\pm$1.3e-03 \\
             & xVAMP &           3.25$\pm$1.16 &           7.6e-03$\pm$3.3e-03 &           5.61$\pm$0.67 &           1.36$\pm$0.14 &           3.2e-03$\pm$5.2e-04 \\
             & xVAMP* &           3.28$\pm$1.17 &           7.6e-03$\pm$3.3e-03 &           5.72$\pm$0.59 &           1.36$\pm$0.14 &           3.2e-03$\pm$4.9e-04 \\
             & VBEM &  \textbf{3.14$\pm$1.07} &           8.7e-03$\pm$3.3e-03 &  \textbf{5.26$\pm$0.58} &           1.36$\pm$0.14 &  \textbf{5.6e-04$\pm$1.6e-04} \\
             & VBEM* &           3.18$\pm$1.12 &           7.6e-03$\pm$3.3e-03 &           5.59$\pm$0.70 &  \textbf{1.30$\pm$0.13} &           2.4e-03$\pm$2.8e-04 \\
\midrule
             &       &             power plant &        superconductivity &                wine-red &              wine-white &                   yacht \\
Algorithm & Prior& (9568, 4, 1)& (21263, 81, 1)& (1599, 11, 1)& (4898, 11, 1)& (308, 6, 1)\\
\midrule
Detlefsen & N/A &           4.33$\pm$0.27 &           17.72$\pm$1.29 &           0.71$\pm$0.06 &           0.76$\pm$0.04 &  \textbf{2.42$\pm$1.06} \\
Normal & N/A &  \textbf{4.12$\pm$0.20} &           14.53$\pm$0.44 &           0.62$\pm$0.03 &           0.70$\pm$0.04 &           3.42$\pm$2.30 \\
Student & N/A &           4.12$\pm$0.19 &           14.85$\pm$0.42 &           0.63$\pm$0.03 &           0.71$\pm$0.03 &          15.03$\pm$3.30 \\
Gamma-Normal & VAP &           4.14$\pm$0.21 &           14.83$\pm$0.48 &           0.62$\pm$0.03 &           0.70$\pm$0.03 &          14.70$\pm$3.31 \\
             & Standard &           4.18$\pm$0.18 &           14.44$\pm$0.43 &           0.63$\pm$0.03 &           0.72$\pm$0.03 &          12.17$\pm$2.38 \\
             & VAMP &           4.16$\pm$0.20 &           12.81$\pm$0.33 &           0.62$\pm$0.03 &           0.70$\pm$0.04 &           5.42$\pm$3.54 \\
             & VAMP* &           4.16$\pm$0.20 &  \textbf{12.80$\pm$0.35} &           0.62$\pm$0.03 &           0.70$\pm$0.04 &           5.30$\pm$3.65 \\
             & xVAMP &           4.14$\pm$0.20 &           14.13$\pm$0.39 &           0.62$\pm$0.03 &           0.70$\pm$0.04 &          12.30$\pm$3.09 \\
             & xVAMP* &           4.13$\pm$0.21 &           14.25$\pm$0.42 &           0.62$\pm$0.03 &           0.70$\pm$0.03 &          12.51$\pm$3.20 \\
             & VBEM &           4.16$\pm$0.19 &           13.13$\pm$0.37 &  \textbf{0.62$\pm$0.03} &  \textbf{0.69$\pm$0.03} &           3.51$\pm$1.46 \\
             & VBEM* &           4.12$\pm$0.19 &           14.08$\pm$0.42 &           0.62$\pm$0.03 &           0.69$\pm$0.03 &           5.33$\pm$2.58 \\
\bottomrule
\end{tabular}



==> assets/regression_uci_sample_bias.tex <==
\begin{tabular}{lllllll}
\toprule
             &       &                   boston &                         carbon &                 concrete &                     energy &                          naval \\
Algorithm & Prior& (506, 13, 1)& (10721, 5, 3)& (1030, 8, 1)& (768, 8, 2)& (11934, 16, 2)\\
\midrule
Detlefsen & N/A &           -0.92$\pm$2.52 &           -9.4e-04$\pm$3.6e-03 &            0.49$\pm$3.93 &              0.17$\pm$1.03 &           -2.6e-04$\pm$6.1e-04 \\
Normal & N/A &  \textbf{-0.19$\pm$0.99} &            4.6e+09$\pm$2.0e+10 &            0.39$\pm$1.05 &              0.06$\pm$0.15 &           -1.2e-04$\pm$1.4e-04 \\
Student & N/A &           -0.58$\pm$0.60 &           -4.3e-05$\pm$1.5e-04 &           -0.14$\pm$1.09 &             -0.07$\pm$0.15 &           -8.3e-05$\pm$2.0e-04 \\
Gamma-Normal & VAP &           -0.34$\pm$0.54 &            1.5e-04$\pm$2.1e-04 &  \textbf{-0.02$\pm$1.18} &             -0.04$\pm$0.14 &  \textbf{-7.0e-06$\pm$1.1e-04} \\
             & Standard &           -0.39$\pm$0.59 &            7.2e-05$\pm$2.9e-04 &            0.04$\pm$1.02 &              0.04$\pm$0.13 &           -1.3e-04$\pm$1.2e-04 \\
             & VAMP &           -0.23$\pm$0.47 &  \textbf{-1.8e-06$\pm$2.9e-04} &           -0.17$\pm$0.83 &              0.01$\pm$0.12 &            7.4e-06$\pm$5.5e-05 \\
             & VAMP* &           -0.24$\pm$0.47 &            6.7e-05$\pm$2.7e-04 &           -0.17$\pm$0.83 &              0.02$\pm$0.12 &            8.2e-06$\pm$5.9e-05 \\
             & xVAMP &           -0.23$\pm$0.69 &           -1.8e-05$\pm$2.4e-04 &           -0.08$\pm$0.88 &           6.0e-03$\pm$0.16 &           -2.2e-05$\pm$1.2e-04 \\
             & xVAMP* &           -0.23$\pm$0.68 &            7.9e-05$\pm$2.6e-04 &           -0.09$\pm$0.97 &  \textbf{2.6e-03$\pm$0.15} &           -1.8e-05$\pm$1.2e-04 \\
             & VBEM &           -0.19$\pm$0.85 &           -4.2e-04$\pm$2.0e-03 &           -0.15$\pm$1.07 &             -0.09$\pm$0.49 &           -2.3e-05$\pm$1.4e-04 \\
             & VBEM* &           -0.24$\pm$0.70 &            3.3e-06$\pm$3.0e-04 &            0.02$\pm$0.79 &              0.02$\pm$0.10 &            1.8e-05$\pm$6.8e-05 \\
\midrule
             &       &                 power plant &       superconductivity &                   wine-red &                  wine-white &                    yacht \\
Algorithm & Prior& (9568, 4, 1)& (21263, 81, 1)& (1599, 11, 1)& (4898, 11, 1)& (308, 6, 1)\\
\midrule
Detlefsen & N/A &               0.12$\pm$0.77 &           1.15$\pm$4.61 &              0.07$\pm$0.18 &           -4.9e-03$\pm$0.08 &           -0.19$\pm$2.16 \\
Normal & N/A &               0.02$\pm$0.16 &     3.6e+04$\pm$1.6e+05 &  \textbf{1.7e-03$\pm$0.08} &            3.8e-03$\pm$0.05 &           -0.70$\pm$1.15 \\
Student & N/A &               0.04$\pm$0.13 &           0.29$\pm$0.61 &             -0.07$\pm$0.08 &              -0.03$\pm$0.04 &           -6.26$\pm$4.34 \\
Gamma-Normal & VAP &  \textbf{-7.6e-03$\pm$0.15} &          -0.06$\pm$0.41 &             -0.02$\pm$0.08 &              -0.02$\pm$0.04 &           -6.16$\pm$4.37 \\
             & Standard &              -0.04$\pm$0.16 &           0.70$\pm$0.51 &             -0.03$\pm$0.08 &              -0.02$\pm$0.04 &           -4.92$\pm$2.49 \\
             & VAMP &              -0.02$\pm$0.13 &           0.16$\pm$0.46 &             -0.02$\pm$0.08 &              -0.02$\pm$0.04 &           -0.62$\pm$1.94 \\
             & VAMP* &              -0.02$\pm$0.13 &           0.14$\pm$0.45 &             -0.02$\pm$0.08 &              -0.02$\pm$0.04 &           -0.58$\pm$1.94 \\
             & xVAMP &              -0.02$\pm$0.18 &          -0.16$\pm$0.62 &             -0.02$\pm$0.08 &              -0.02$\pm$0.04 &           -5.13$\pm$2.98 \\
             & xVAMP* &              -0.02$\pm$0.15 &          -0.13$\pm$0.62 &             -0.02$\pm$0.08 &              -0.02$\pm$0.04 &           -5.36$\pm$3.12 \\
             & VBEM &              -0.04$\pm$0.21 &           0.10$\pm$0.67 &             -0.02$\pm$0.08 &              -0.01$\pm$0.04 &  \textbf{-0.19$\pm$0.89} \\
             & VBEM* &               0.04$\pm$0.15 &  \textbf{0.04$\pm$0.57} &          -7.3e-03$\pm$0.06 &  \textbf{-2.3e-03$\pm$0.04} &           -1.74$\pm$1.59 \\
\bottomrule
\end{tabular}



==> assets/regression_uci_sample_rmse.tex <==
\begin{tabular}{lllllll}
\toprule
             &       &                  boston &                        carbon &                concrete &                  energy &                         naval \\
Algorithm & Prior& (506, 13, 1)& (10721, 5, 3)& (1030, 8, 1)& (768, 8, 2)& (11934, 16, 2)\\
\midrule
Detlefsen & N/A &          12.02$\pm$3.89 &              0.03$\pm$3.6e-03 &          17.93$\pm$2.55 &           5.07$\pm$0.98 &           6.2e-03$\pm$5.7e-04 \\
Normal & N/A &           4.92$\pm$3.57 &           2.6e+11$\pm$1.2e+12 &           8.23$\pm$1.08 &  \textbf{1.85$\pm$0.21} &           5.0e-03$\pm$5.4e-04 \\
Student & N/A &           4.64$\pm$1.10 &  \textbf{8.1e-03$\pm$3.1e-03} &           9.18$\pm$1.36 &           2.07$\pm$0.37 &           5.0e-03$\pm$1.7e-03 \\
Gamma-Normal & VAP &           4.69$\pm$0.86 &              0.01$\pm$2.2e-03 &           9.42$\pm$1.82 &           2.02$\pm$0.35 &           4.5e-03$\pm$7.2e-04 \\
             & Standard &           4.92$\pm$2.18 &              0.02$\pm$1.8e-03 &           8.67$\pm$1.20 &           1.88$\pm$0.38 &           4.6e-03$\pm$9.1e-04 \\
             & VAMP &           4.27$\pm$0.87 &              0.01$\pm$1.9e-03 &           7.27$\pm$1.05 &           1.93$\pm$0.19 &  \textbf{1.8e-03$\pm$1.4e-03} \\
             & VAMP* &           4.26$\pm$0.86 &              0.01$\pm$2.0e-03 &  \textbf{7.27$\pm$1.05} &           1.93$\pm$0.20 &           2.2e-03$\pm$1.8e-03 \\
             & xVAMP &  \textbf{4.23$\pm$1.15} &              0.01$\pm$2.0e-03 &           7.84$\pm$1.05 &           1.88$\pm$0.29 &           4.5e-03$\pm$7.5e-04 \\
             & xVAMP* &           4.23$\pm$1.14 &              0.01$\pm$2.5e-03 &           8.00$\pm$1.01 &           1.87$\pm$0.30 &           4.5e-03$\pm$7.1e-04 \\
             & VBEM &           5.03$\pm$0.92 &                 0.11$\pm$0.03 &           9.21$\pm$0.98 &           5.13$\pm$0.83 &           5.9e-03$\pm$1.5e-03 \\
             & VBEM* &           4.41$\pm$1.07 &              0.01$\pm$1.9e-03 &           7.90$\pm$1.10 &           1.85$\pm$0.30 &           3.5e-03$\pm$3.7e-04 \\
\midrule
             &       &             power plant &        superconductivity &                wine-red &              wine-white &                   yacht \\
Algorithm & Prior& (9568, 4, 1)& (21263, 81, 1)& (1599, 11, 1)& (4898, 11, 1)& (308, 6, 1)\\
\midrule
Detlefsen & N/A &          10.36$\pm$0.28 &        2.4e+02$\pm$15.98 &           1.43$\pm$0.34 &           1.27$\pm$0.10 &          10.71$\pm$2.19 \\
Normal & N/A &           5.85$\pm$0.20 &      1.7e+06$\pm$7.4e+06 &  \textbf{0.86$\pm$0.07} &           0.98$\pm$0.03 &  \textbf{4.73$\pm$3.68} \\
Student & N/A &  \textbf{5.79$\pm$0.28} &           21.25$\pm$1.46 &           0.88$\pm$0.06 &           0.99$\pm$0.04 &          20.24$\pm$7.84 \\
Gamma-Normal & VAP &           5.90$\pm$0.26 &           21.05$\pm$0.81 &           0.89$\pm$0.06 &           0.99$\pm$0.04 &          20.00$\pm$7.47 \\
             & Standard &           6.01$\pm$0.51 &          23.75$\pm$13.27 &           0.90$\pm$0.13 &           0.98$\pm$0.06 &          14.20$\pm$4.40 \\
             & VAMP &           5.97$\pm$0.28 &           17.86$\pm$0.41 &           0.90$\pm$0.07 &           0.99$\pm$0.06 &           8.67$\pm$6.43 \\
             & VAMP* &           5.97$\pm$0.28 &  \textbf{17.85$\pm$0.42} &           0.90$\pm$0.07 &           0.99$\pm$0.06 &           8.50$\pm$6.57 \\
             & xVAMP &           5.92$\pm$0.20 &           19.98$\pm$0.49 &           0.89$\pm$0.05 &  \textbf{0.97$\pm$0.06} &          15.57$\pm$5.76 \\
             & xVAMP* &           5.91$\pm$0.20 &           20.19$\pm$0.77 &           0.89$\pm$0.05 &           0.97$\pm$0.06 &          15.81$\pm$5.05 \\
             & VBEM &           7.17$\pm$0.65 &           20.92$\pm$0.70 &           0.93$\pm$0.06 &           1.02$\pm$0.05 &           6.66$\pm$2.53 \\
             & VBEM* &           6.00$\pm$0.20 &           19.78$\pm$0.48 &           0.89$\pm$0.07 &           0.97$\pm$0.03 &           6.84$\pm$4.58 \\
\bottomrule
\end{tabular}



==> assets/regression_uci_var_bias.tex <==
\begin{tabular}{lllllll}
\toprule
             &       &                   boston &                         carbon &                 concrete &                     energy &                         naval \\
Algorithm & Prior& (506, 13, 1)& (10721, 5, 3)& (1030, 8, 1)& (768, 8, 2)& (11934, 16, 2)\\
\midrule
Detlefsen & N/A &        1.0e+02$\pm$79.11 &            9.8e-05$\pm$1.6e-04 &        2.2e+02$\pm$91.85 &             18.60$\pm$8.88 &                   nan$\pm$nan \\
Normal & N/A &        31.63$\pm$1.5e+02 &            3.5e+23$\pm$1.6e+24 &           -2.01$\pm$8.67 &             -0.16$\pm$0.24 &           3.1e-07$\pm$2.0e-06 \\
Student & N/A &          18.08$\pm$63.79 &                  0.12$\pm$0.23 &           -2.20$\pm$9.28 &            24.00$\pm$85.42 &           4.9e-06$\pm$2.2e-05 \\
Gamma-Normal & VAP &      3.3e+02$\pm$1.3e+03 &                  0.25$\pm$1.11 &           -2.13$\pm$7.85 &              0.04$\pm$0.31 &           3.1e-07$\pm$6.8e-07 \\
             & Standard &           3.18$\pm$20.09 &            1.5e-04$\pm$5.8e-05 &           0.76$\pm$11.35 &              0.31$\pm$0.40 &           3.7e-06$\pm$2.9e-06 \\
             & VAMP &           -2.96$\pm$7.96 &           -6.6e-06$\pm$6.0e-05 &           -6.15$\pm$5.18 &             -0.15$\pm$0.39 &           1.7e-07$\pm$2.9e-07 \\
             & VAMP* &           -3.00$\pm$7.84 &  \textbf{-6.0e-06$\pm$6.0e-05} &           -6.16$\pm$5.18 &             -0.13$\pm$0.40 &  \textbf{1.3e-07$\pm$3.3e-07} \\
             & xVAMP &           0.65$\pm$16.20 &            2.7e-05$\pm$9.7e-05 &           -4.82$\pm$4.63 &  \textbf{6.0e-03$\pm$0.36} &           3.1e-07$\pm$7.4e-07 \\
             & xVAMP* &           0.51$\pm$20.17 &            5.0e-04$\pm$2.2e-03 &           -4.66$\pm$5.07 &          -8.5e-03$\pm$0.36 &           2.7e-07$\pm$6.3e-07 \\
             & VBEM &            6.74$\pm$8.48 &               0.01$\pm$4.5e-03 &           25.86$\pm$8.94 &             22.06$\pm$5.58 &           3.6e-05$\pm$1.4e-05 \\
             & VBEM* &  \textbf{-0.11$\pm$8.62} &           -7.2e-06$\pm$6.1e-05 &  \textbf{-0.58$\pm$5.05} &              0.02$\pm$0.28 &           3.9e-07$\pm$4.9e-07 \\
\midrule
             &       &             power plant &        superconductivity &                   wine-red &                  wine-white &                     yacht \\
Algorithm & Prior& (9568, 4, 1)& (21263, 81, 1)& (1599, 11, 1)& (4898, 11, 1)& (308, 6, 1)\\
\midrule
Detlefsen & N/A &          69.25$\pm$2.40 &      5.5e+04$\pm$6.2e+03 &              2.16$\pm$1.57 &               0.83$\pm$0.36 &           96.62$\pm$54.08 \\
Normal & N/A &  \textbf{0.05$\pm$1.53} &      2.3e+13$\pm$1.0e+14 &          -3.8e-03$\pm$0.04 &              -0.02$\pm$0.06 &           20.68$\pm$54.95 \\
Student & N/A &          -0.27$\pm$1.47 &      1.6e+05$\pm$3.3e+05 &            12.52$\pm$30.71 &           -5.6e-03$\pm$0.05 &       1.7e+03$\pm$2.3e+03 \\
Gamma-Normal & VAP &           0.52$\pm$1.29 &      9.0e+05$\pm$2.6e+06 &              0.03$\pm$0.05 &               0.13$\pm$0.64 &       1.3e+03$\pm$1.5e+03 \\
             & Standard &           2.34$\pm$1.43 &        1.1e+02$\pm$81.21 &              0.04$\pm$0.11 &  \textbf{-2.3e-03$\pm$0.05} &  \textbf{-7.28$\pm$40.88} \\
             & VAMP &           0.89$\pm$1.04 &  \textbf{-9.83$\pm$7.97} &              0.05$\pm$0.06 &           -8.8e-03$\pm$0.04 &           38.05$\pm$83.39 \\
             & VAMP* &           0.89$\pm$1.04 &           -9.89$\pm$7.98 &              0.05$\pm$0.06 &           -8.9e-03$\pm$0.04 &           38.07$\pm$83.29 \\
             & xVAMP &           0.46$\pm$1.25 &          14.40$\pm$42.90 &           3.5e-03$\pm$0.05 &              -0.03$\pm$0.03 &       4.8e+02$\pm$1.7e+03 \\
             & xVAMP* &           0.44$\pm$1.24 &      1.3e+02$\pm$4.7e+02 &  \textbf{2.1e-03$\pm$0.05} &              -0.03$\pm$0.03 &       1.7e+02$\pm$1.5e+02 \\
             & VBEM &          16.53$\pm$9.32 &          91.44$\pm$25.39 &              0.08$\pm$0.04 &               0.07$\pm$0.04 &           20.70$\pm$25.23 \\
             & VBEM* &           1.86$\pm$1.44 &           9.87$\pm$16.22 &              0.05$\pm$0.06 &               0.01$\pm$0.04 &           26.48$\pm$26.88 \\
\bottomrule
\end{tabular}



==> assets/regression_uci_var_rmse.tex <==
\begin{tabular}{lllllll}
\toprule
             &       &                    boston &                        carbon &                  concrete &                  energy &                         naval \\
Algorithm & Prior& (506, 13, 1)& (10721, 5, 3)& (1030, 8, 1)& (768, 8, 2)& (11934, 16, 2)\\
\midrule
Detlefsen & N/A &       2.5e+02$\pm$3.1e+02 &           2.8e-03$\pm$1.8e-03 &       2.9e+02$\pm$1.1e+02 &         21.58$\pm$10.55 &                   nan$\pm$nan \\
Normal & N/A &       2.8e+02$\pm$1.1e+03 &           2.0e+25$\pm$8.8e+25 &           84.48$\pm$46.55 &  \textbf{2.70$\pm$0.50} &           3.6e-05$\pm$1.5e-05 \\
Student & N/A &       1.1e+02$\pm$1.7e+02 &                 1.19$\pm$2.12 &           86.73$\pm$25.52 &     1.0e+02$\pm$3.6e+02 &           1.4e-04$\pm$4.8e-04 \\
Gamma-Normal & VAP &       2.4e+03$\pm$9.5e+03 &                4.74$\pm$20.81 &           80.57$\pm$26.95 &           3.64$\pm$1.10 &           2.3e-05$\pm$8.7e-06 \\
             & Standard &           76.10$\pm$83.67 &           2.8e-03$\pm$1.8e-03 &           92.78$\pm$28.09 &           3.05$\pm$1.00 &           3.0e-05$\pm$1.1e-05 \\
             & VAMP &           31.89$\pm$37.72 &  \textbf{2.7e-03$\pm$1.9e-03} &           60.50$\pm$29.84 &           4.19$\pm$0.79 &  \textbf{5.5e-06$\pm$7.0e-06} \\
             & VAMP* &  \textbf{31.82$\pm$37.33} &           2.7e-03$\pm$1.9e-03 &           60.49$\pm$29.84 &           4.19$\pm$0.79 &           7.8e-06$\pm$9.1e-06 \\
             & xVAMP &           63.40$\pm$84.86 &           3.0e-03$\pm$1.7e-03 &           59.74$\pm$20.73 &           3.36$\pm$0.88 &           2.3e-05$\pm$8.7e-06 \\
             & xVAMP* &         64.27$\pm$1.2e+02 &                 0.02$\pm$0.05 &           62.39$\pm$19.00 &           3.19$\pm$0.78 &           2.2e-05$\pm$6.3e-06 \\
             & VBEM &           38.91$\pm$35.36 &              0.01$\pm$4.3e-03 &           59.36$\pm$13.87 &          26.09$\pm$6.92 &           4.2e-05$\pm$1.6e-05 \\
             & VBEM* &           39.54$\pm$42.93 &           2.8e-03$\pm$1.9e-03 &  \textbf{58.92$\pm$19.43} &           3.72$\pm$0.47 &           1.5e-05$\pm$3.8e-06 \\
\midrule
             &       &               power plant &           superconductivity &                wine-red &              wine-white &                     yacht \\
Algorithm & Prior& (9568, 4, 1)& (21263, 81, 1)& (1599, 11, 1)& (4898, 11, 1)& (308, 6, 1)\\
\midrule
Detlefsen & N/A &           85.20$\pm$10.25 &         2.2e+05$\pm$1.7e+04 &           7.27$\pm$9.73 &           2.91$\pm$3.65 &         1.1e+02$\pm$70.70 \\
Normal & N/A &  \textbf{43.93$\pm$18.42} &         1.1e+15$\pm$4.8e+15 &           0.63$\pm$0.09 &           1.05$\pm$0.82 &       1.2e+02$\pm$2.7e+02 \\
Student & N/A &           44.88$\pm$18.75 &         5.8e+06$\pm$1.3e+07 &     1.2e+02$\pm$3.4e+02 &           0.96$\pm$0.35 &       5.7e+03$\pm$8.2e+03 \\
Gamma-Normal & VAP &           44.40$\pm$18.82 &         4.0e+07$\pm$1.2e+08 &           0.65$\pm$0.10 &          3.97$\pm$13.91 &       4.8e+03$\pm$5.7e+03 \\
             & Standard &           45.18$\pm$18.49 &         1.5e+03$\pm$1.7e+03 &           0.77$\pm$0.38 &           0.94$\pm$0.20 &         1.1e+02$\pm$66.59 \\
             & VAMP &           44.78$\pm$18.79 &  \textbf{4.4e+02$\pm$55.55} &           0.63$\pm$0.09 &           0.87$\pm$0.25 &         99.44$\pm$1.2e+02 \\
             & VAMP* &           44.78$\pm$18.79 &           4.4e+02$\pm$57.11 &           0.63$\pm$0.09 &           0.87$\pm$0.25 &         98.63$\pm$1.3e+02 \\
             & xVAMP &           44.44$\pm$18.84 &         1.1e+03$\pm$1.8e+03 &  \textbf{0.63$\pm$0.11} &           0.85$\pm$0.23 &       1.4e+03$\pm$4.8e+03 \\
             & xVAMP* &           44.36$\pm$18.82 &         6.4e+03$\pm$2.1e+04 &           0.63$\pm$0.11 &           0.85$\pm$0.23 &       5.6e+02$\pm$4.9e+02 \\
             & VBEM &           49.60$\pm$16.88 &           4.5e+02$\pm$59.88 &           0.63$\pm$0.11 &  \textbf{0.82$\pm$0.11} &  \textbf{39.19$\pm$37.73} \\
             & VBEM* &           44.68$\pm$18.61 &         6.3e+02$\pm$4.2e+02 &           0.64$\pm$0.10 &           0.86$\pm$0.28 &           93.02$\pm$86.57 \\
\bottomrule
\end{tabular}


